Buy-many mechanisms are not much better than item pricing

Multi-item mechanisms can be very complex offering many different bundles to the buyer that could even be randomized. Such complexity is thought to be necessary as the revenue gaps between randomized and deterministic mechanisms, or deterministic and simple mechanisms are huge even for additive valuations. We challenge this conventional belief by showing that these large gaps can only happen in restricted situations. These are situations where the mechanism overcharges a buyer for a bundle while selling individual items at much lower prices. Arguably this is impractical in many settings because the buyer can break his order into smaller pieces paying a much lower price overall. Our main result is that if the buyer is allowed to purchase as many (randomized) bundles as he pleases, the revenue of any multi-item mechanism is at most O(logn) times the revenue achievable by item pricing, where n is the number of items. This holds in the most general setting possible, with an arbitrarily correlated distribution of buyer types and arbitrary valuations. We also show that this result is tight in a very strong sense. Any family of mechanisms of subexponential description complexity cannot achieve better than logarithmic approximation even against the best deterministic mechanism and even for additive valuations. In contrast, item pricing that has linear description complexity matches this bound against randomized mechanisms.

==> simpledistribution.tex <==
\section{A constant upper bound for special demand distributions}

In the previous section we proved that we cannot obtain an $o(\log n)$-approximation to deterministic subadditive pricing via simple mechanisms for arbitrary distributions over valuation functions. However, when the distributions satisfy a certain property simple mechanisms, in particular item or bundle pricings, are able to do better.

\begin{definition}
  Given a deterministic Sybil-proof pricing $p$ and a distribution $\dist$ over valuations, the {\em demand distribution} $\Pi_{p,\dist}$ is the distribution over sets of items that specifies the random set of items bought by a buyer with value drawn from $\dist$ under pricing $p$: for all $S\subseteq [n]$, $\Pi_{p,\dist}(S) = \Pr_{v\sim\dist}[S = \argmax_{T\subseteq [n]} (v(T)-p(T))]$.\footnote{Generally speaking, specifying the demand distribution requires specifying a tie-breaking rule between multiple sets of equal utility. We will focus here on single-minded buyers, so the possibility of tie-breaking will not arise.}
\end{definition}

Observe that for any pricing $p$ and value distribution $\dist$, the revenue of the pricing is precisely $\expect[v\sim\dist]{p(v)} = \expect[S\sim\Pi_{p,\dist}]{p(S)}$. We will now show that if the buyer is single-minded and the demand distribution is a product distribution over items, then the revenue of $p$ can be approximated by a simple pricing.

% Let $f:\{0,1\}^n\to\R_0^+$ be a deterministic subadditive pricing function over sets. Assume that given such pricing, the set of items purchased by the buyer follows product distribution $\Pi$, where each item $i$ is purchased independently with probability $\pi_i$. While the subadditive function can be complicated, we prove that simple mechanism can get comparable revenue. To be more precise, either item pricing or grand bundle pricing is constant approximation of the revenue of pricing $f$.
\begin{theorem}
Given a deterministic monotone subadditive pricing function $p$ and value distribution $\dist$ over single-minded values, suppose that the demand distribution $\Pi_{p,\dist}$ is a product distribution over items, then $\rev_\dist(p)< 22.67\max(\srev_\dist,\brev_\dist)$.
\end{theorem}
\begin{proof}
As in the work of \cite{rw-15}, we will break up set of items and correspondingly the revenue obtained by $p$ into two components: over one of these components, a.k.a. the core, the price will concentrate around its expectation and can be approximated using a bundle pricing; over the other, a.k.a. the tail, a significant fraction of the revenue will be contributed by singleton items and can be recovered using an item pricing.

We write $\Pi$ as shorthand for $\Pi_{p,\dist}$. Number the items in decreasing order of their individual prices: $p(\{1\})\geq p(\{2\})\geq\cdots\geq p(\{n\})$. For items $i\in [n]$ let $\pi_i$ denote the marginal probability that $i$ is purchased, that is, $\pi_i = \Pr_{S\sim\Pi}[i\in S]$. Find the index $k\in[n]$ such that $\pi_1+\pi_2+\cdots+\pi_{k}<\frac{1}{2}$ and $\pi_1+\pi_2+\cdots+\pi_{k+1}\geq\frac{1}{2}$. The high value, low probability items $\{1, 2, \cdots, k\}$ will form the tail, and the remaining items will form the core.
%Based on the value of $\pi_{k+1}$, we have the following two cases. 
For any subset $S\subseteq [n]$, define $S_{\tail}=S\cap\{1,2,\cdots,k\}$ and $S_{\core}=S\cap\{k+1,\cdots,n\}$. By the subadditivity of $p$ we have $p(S)\leq p(S_{\tail})+p(S_{\core})$. Therefore, $\expect[S\sim\Pi]{p(S_{\tail})}+\expect[S\sim\Pi]{p(S_{\core})}$ is an upper bound of the revenue of $p$.

We will first bound the contribution of the core, $\expect[S\sim\Pi]{p(S_{\core})}$ using the following concentration lemma for subadditive functions from \cite{schechtman2003concentration}. To apply the lemma, we observe that $p(S_{\core})$ is Lipschitz with a Lipschitz constant of $\max_{i>k} p(\{i\}) = p(\{k+1\})$ because $S_{\core}$ contains only items with index larger than $k$.  
% Partition set $S$ purchased by the buyer into two parts: $S_{\tail}=S\cap\{1,2,\cdots,k+1\}$, and $S_{\core}=S\cap\{k+2,\cdots,n\}$. Since the pricing function $p$ is subadditive, for any set $S\subseteq [n]$, $f(S)\leq f(S_{\tail})+f(S_{\core})$. Thus $\expect{f(S_{\tail})}+\expect{f(S_{\core})}$ is an upper bound of the revenue of subadditive pricing. Let $c=f(\{k+1\})$. Since all items are sorted in decreasing order of the value of singleton sets, we observe that $f(S_{\core})$ is $c$-Lipschitz, since $S_{\core}$ contains only items with index larger than $k+2$. Similar to the approach in \cite{rw-15}, we apply the following concentration result on subadditive functions from \cite{schechtman2003concentration}.
\begin{theorem}
(Corollary 12 from \cite{schechtman2003concentration}) Suppose that $f(X)$ is a non-negative $c$-Lipschitz subadditive function, where $X\in\{0,1\}^n$ is drawn from a product distribution $D$. If $a$ is the median of $f$, then for any $k>0$, $\Pr_{X\sim D}[f(X)\geq 3a+k]\leq 2^{2-k/c}$.
\end{theorem}
Setting $a = \operatorname{median}_{S\sim\Pi}(p(S_\core))$ and $c=p(\{k+1\})$, we obtain
%Let $a$ be the median of $f(S_\core)$. Notice that
\[\expect[S\sim\Pi]{p(S_{\core})}=\int_{t\geq 0}\Pr[p(S_{\core})>t]dt\leq 3a+\int_{k\geq0}2^{2-k/c}dk=3a+\frac{4}{\ln 2}c.\]
We now observe that we can recover both of the terms above using a bundle pricing. In particular, by setting a constant bundle price of $a$, we obtain a revenue of  $a\Pr_{v\sim\dist} [v([n])>a] \ge a\Pr_{S\sim\Pi} [p(S)>a] \ge a\Pr_{S\sim\Pi} [p(S_\core)>a] = a/2$. On the other hand, by setting a constant bundle price of $c$, we obtain a revenue of $c\Pr_{v\sim\dist} [v([n])>c] \ge c\Pr_{S\sim\Pi} [p(S)>c] \ge c\Pr_{S\sim\Pi}[\exists i\le k+1: i\in S]$. The latter probability can be bounded from below as:
% Since $a$ is the median of $f(S_\core)$, consider a mechanism that sells the entire bundle of $n$ items at price $a$, then the revenue achieved by such mechanism is $\frac{1}{2}a$, which implies $\brev\geq\frac{1}{2}a$. Since $c=f(\{k+1\})$, then for every set $S$, if $S$ contains an item with index at most $k+1$, then $f(S)\geq c$. Consider a mechanism that sells the entire bundle of $n$ items at price $c$, then the probability of sell is at least
\[\Pr_{S\sim\Pi}[\exists i\leq k+1,\ i\in S]=1-(1-\pi_1)(1-\pi_2)\cdots(1-\pi_{k+1})\geq 1-\left(1-\frac{\sum_{i\leq k+1}\pi_i}{k+1}\right)^{k+1}\geq1-e^{-1/2},\]
where the first inequality follows by applying Jensen's inequality, and the second follows by using $\sum_{i\leq k+1}\pi_i\geq\frac{1}{2}$. 

%Thus the revenue collected from the bundling pricing mechanism is at least $(1-e^{-1/3})c$, which implies $\brev\geq (1-e^{-1/3})c$. 
Thus we can bound $\expect{p(S_\core)}$ as follows:
\[\expect{p(S_{\core})}\leq3a+\frac{4}{\ln 2}c\leq 6\,\brev+\frac{4}{(1-e^{-1/2})\ln 2}\brev< 20.67\,\brev.\]

Now we bound $\expect{p(S_\tail)}$. By subadditivity, 
\[\expect{p(S_\tail)}\leq\expect{\sum_{i\leq k}p(S_\tail\cap\{i\})}=\sum_{i\leq k}\pi_ip(\{i\}).\] 
Recall that $\pi_1+\pi_2+\cdots+\pi_{k}\leq\frac{1}{2}$. Consider the additive pricing that sells items in $\{1,2,\cdots,k\}$ at item prices $q_i=p(\{i\})$, and allocates items $i>k$ for free.

Consider a buyer that purchases a set $S$ under pricing $p$ with $S_\tail=\{i\}$. In the pricing $q$, the buyer continues to afford the set $S$ at a lower price of $q_i=p(\{i\})<p(S)$. Therefore, the revenue of the pricing $q$ from this buyer is at least $q_i=p(\{i\})$. Since this buyer is instantiated with probability at least $\Pr[S_\tail=\{i\}] \ge \frac 12 \pi_i$, we get that $\expect{p(S_\tail)}\leq 2\,\rev_\dist(q)\le 2\,\srev$. Then combining the above cases we get $\rev_\dist(p)\leq 22.67\max(\srev_\dist,\brev_\dist)$.
\end{proof} 
% For any item $i$, if $i\in S_\tail$, then by union bound with probability at most $\frac{1}{3}$ non of other items appear in $S_\tail$. Thus the revenue is at least $\frac{1}{3}\sum_{i\leq k+1}\pi_i p_i\geq\frac{1}{3}\expect{f(S_\tail)}$, which implies $\expect{f(S_{\tail})}\leq 3\srev$.
% If $\pi_1+\pi_2+\cdots+\pi_{k+1}>\frac{2}{3}$, then $\pi_{k+1}>\frac{1}{3}$. Consider the following two mechanisms: the first mechanism sells each item in $\{1,2,\cdots,k\}$ separately, with item price $p_i=f(\{i\})$ for item $i\leq k$. The second mechanism sells the grand bundle at price $f(\{k+1\})$. The same as above we can show that the revenue of the first mechanism is at least $\frac{2}{3}\sum_{i\leq k}\pi_i p_i$, while the second mechanism has sell probability at least $\pi_{k+1}$ and revenue at least $\pi_{k+1}f(\{k+1\})$. Thus $\expect{f(S_\tail)}\leq\sum_{i\leq k+1}\pi_if(\{i\})\leq\frac{3}{2}\srev+\brev$.


